Lagrangian Approximations for Stochastic Reachability of a Target Tube

In this paper we examine how Lagrangian techniques can be used to compute underapproximations and overapproximation of the finite-time horizon, stochastic reach-avoid level sets for discrete-time, nonlinear systems. This approach is applicable for a generic nonlinear system without any convexity assumptions on the safe and target sets. We examine and apply our methods on the reachability of a target tube problem, a more generalized version of the finite-time horizon reach-avoid problem. Because these methods utilize a Lagrangian (set theoretic) approach, we eliminate the necessity to grid the state, input, and disturbance spaces allowing for increased scalability and faster computation. The methods scalability are currently limited by the computational requirements for performing the necessary set operations by current computational geometry tools. The primary trade-off for this improved extensibility is conservative approximations of actual stochastic reach set. We demonstrate these methods on several examples including the standard double-integrator, a chain of integrators, and a 4-dimensional space vehicle rendezvous docking problem.

==> cutout.tex <==
\subsection{Bertsekas formulation}


\begin{figure*}[t!]
    \begin{align}
        V_{N-t}^\ast(x)
        &= \mathbb{P}^{t,\pi^\ast}_{\bar{x}_{t}}(x_{N} \in \mathcal{T}, x_{N-1}
        \in \mathcal{K}, \dots, x_{N-t+1} \in \mathcal{K} | x)\ONE_{ \mathcal{K}}(x)  \nonumber \\
                 &= \mathbb{P}^{t,\pi^\ast}_{\bar{x}_{t}}(x_{N} \in \mathcal{T}, x_{N-1}
        \in \mathcal{K}, \dots, x_{N-t+1} \in \mathcal{K} | x, \bar{w}_{t}\in \boundeddist^{t})  \mathbb{P}_{\bar{w}_{t}}^{t}(\bar{w}_{t}\in \boundeddist^{t}) \nonumber \\
                 &\qquad+\mathbb{P}^{t,\pi^\ast}_{\bar{x}_{t}}(x_{N}
        \in \mathcal{T}, x_{N-1} \in \mathcal{K}, \dots, x_{N-t+1} \in \mathcal{K} | x, \bar{w}_{t}\in (\mathcal{W}^{t}\setminus\boundeddist^{t})) \mathbb{P}_{\bar{w}_{t}}^{t}(\bar{w}_{t}\in
        (\mathcal{W}^{t}\setminus\boundeddist^{t}))\label{eq:totProb}\\
        &\geq  \mathbb{P}^{t,\pi^\ast}_{\bar{x}_{t}}(x_{N} \in \mathcal{T}, x_{N-1}
        \in \mathcal{K}, \dots,  x_{N-t+1} \in \mathcal{K} | x, \bar{w}_{t}\in \boundeddist^{t}) \mathbb{P}_{\bar{w}_{t}}^{t}(\bar{w}_{t}\in
        \boundeddist^{t}).\label{eq:LowerBound} 
           %&= \sum_{\bar{v} \in
    %\mathcal{D}^{N-k}}\mathbb{P}^{k,\pi^\ast}_{\bar{x}_{k}}(x_{N} \in T, x_{N-1} \in K, \dots, x_{k+1} \in K | x, \bar{v})
    %\mathbb{P}_{\bar{w}_{k}}^k(\bar{w}_{k}=\bar{v}) \nonumber \\
    %&+\sum_{\bar{v} \in
    %(\mathcal{W}^{N-k}\setminus\mathcal{D}^{N-k})}\mathbb{P}^{k,\pi^\ast}_{\bar{x}_{k}}(x_{N}
    %\in T, x_{N-1} \in K, \dots, x_{k+1} \in K | x, \bar{v})
    %\mathbb{P}_{\bar{w}_{k}}^k(\bar{w}_{k}=\bar{v}).\label{eq:totProb}
    \end{align}
    \hrulefill
\end{figure*}


\subsection{Recursion for computation of robust effective target set}


As in~\cite{maidens_2013,GleasonCDC2017}, we define the unperturbed, one-step forward reach set from a point $x\in \statespace$ for the system \eqref{eq:nonlin-dist} as $\reachf(x)$, and the unperturbed, one-step backward reach set from a set $ \mathcal{S} \subseteq \statespace$ as $\reachd(\mathcal{S})$. 
Formally, for the system \eqref{eq:nonlin-dist},
\begin{align}
    \reachf(x) &\triangleq \{ x^+\in \statespace : \exists u \in \inputspace,\ x^+=f(x,u)\}\label{eq:reachF}\\
    \reachd(\mathcal{S})&\triangleq\left\{ x^- \in \statespace : \exists u\in
\inputspace, \exists y\in \mathcal{S},\ y=f(x^-,u)\right\} \nonumber \\ %\label{eq:dr1-set}\\
&=\left\{ x^- \in \statespace : \reachf(x^-)\cap \mathcal{S}\neq\emptyset
\right\} \label{eq:dFcapS}
\end{align}
%where \eqref{eq:dFcapS} follows from \eqref{eq:reachF}.  
For an LTI system \eqref{eq:lin}, these can be written as 
\begin{align}
    \reachf(x)&=A\{x\}\oplus B \inputspace,\label{eq:FOlin} \\
    \reachd( \mathcal{S})&= A^{-1}(\mathcal{S}\oplus (-B
    \inputspace)).\label{eq:reachOlinCts}
\end{align}
% \begin{itemize}
% \item Figure~\ref{fig:ProbSt}.
% \item See Problem 8.28 for containment of polytopes as a LP
% \item Volume of a polyhedron is a log-concave function of b when the polyhedron is described is $Ax\leq b$. Example 3.44 in Boyd.
% \end{itemize}

With these definitions we can establish a recursion for the exact computation of the robust effective target set.
\begin{theorem}\label{thm:robust-effective-target-recursion}
  For the system given in (\ref{eq:nonlin-dist}), the finite-time robust reach-avoid sets $\radfull{k}$ can be computed using the recursion  for $k\geq 1,k\in \mathbb{N}$:
  \begin{align}
      \rad_{N}(\targettube_{N},\boundeddist) &= \targetset_{N}
      \label{eq:dra_recurse0}\\
      \rad_{k}(\targettube_{N},\boundeddist) &= \targetset_{k} \cap \reachd(\rad_{k+1}( \targettube_{N},\boundeddist) \minkdiff \boundeddist)\label{eq:dra_recursen}
  \end{align}
\end{theorem}
\begin{proof}
    We prove this by induction. Starting with the base case, $k=N-1$,
    \begin{align}
        \targetset_{N-1} \,\cap\, & \reachd(\radfull{N} \minkdiff \boundeddist) \nonumber \\
        & = \targetset_{N-1} \cap\, \reachd(\targetset_{N} \ominus \boundeddist) \\
        & = \targetset_{N-1} \cap\, \big\{x^{-} \in \statespace : \exists \nu \in \mathcal{F}, \forall w_{N-1} \in \boundeddist \nonumber \\
        & \hskip2cm f(x^{-}, \nu(x^{-})) + w_{N-1} \in \targetset_{N} \big\} \\
        & = \big\{ x_{N-1} \in \targetset_{N-1}: \exists \nu_{N-1} \in \mathcal{F}, \forall w_{N-1} \in \boundeddist, \nonumber \\
        & \hskip2cm f(x_{N-1}, \nu(x_{N-1})) + w_{N-1} \in \targetset_{N} \big\} \\
        & = \big\{ x_{N-1} \in \targetset_{N-1} : \exists \nu_{N-1} \in \mathcal{F}, \forall w_{N-1} \in \boundeddist, \nonumber \\
        & \hskip3.2cm x_{N} \in \targetset_{N} \big\} \\
        & = \radfull{N-1}.
    \end{align}
    For any $k \in \naturalnums$, $k < N-1$
    % , see equations 
    % \eqref{eq:recursion-k-start}--\eqref{eq:recursion-k-end}.
    \begin{align}
        \targetset_{k} \,\cap\, &\reachd(\radfull{k+1} \minkdiff \boundeddist) \nonumber \\
        & = \big\{ x_{k} \in \targetset_{k}: \exists \nu_{k} \in \mathcal{F}, \forall w_{k} \in \boundeddist, \nonumber \\
        & \hskip1.5cm f(x_{k}, \nu(x_{k})) + w_{k} \in \radfull{k+1} \big\} \label{eq:recursion-k-start}\\
        & = \big\{ x_{k} \in \targetset_{k} : \exists \nu_{k} \in \mathcal{F}, \forall w_{k} \in \boundeddist,  \nonumber \\
        & \hskip1.5cm x_{k+1} \in \radfull{k+1} \big\}.
    \end{align}
    By expanding $\radfull{k+1}$ with its definition \eqref{eq:robust-effective-target-set},
    \begin{align}
        % \phantom{\hbox to 0.8cm{}} &= \left\{ x_{k} \in \mathcal{K} : \exists \nu_{k} \in \mathcal{F}, \forall w_{N-1} \in \boundeddist,  x_{k+1}, \in \left\{x_{t+1} \in \mathcal{K}:
        % \begin{array}{l}
        %     \exists \nu_{t+1}\in \mathcal{F}, \forall w_{t+1}\in \boundeddist, x_{t+2} \in \mathcal{K}, \\
        %     \hfill\vdots\hfill \\
        %     \exists \nu_{N-1}\in \mathcal{F}, \forall w_{N-1}\in \boundeddist, x_{N} \in \mathcal{T} \\
        % \end{array}\right\}\right\} \\
         &= \big\{  x_{k} \in \mathcal{K} : \forall t \in \dtinterval{k}{N-1}, \exists \nu_{t} \in \mathcal{F}, \hskip0.6cm \nonumber \\
        & \hskip2.04cm \forall w_{t} \in \boundeddist, x_{t+1} \in \targetset_{t+1} \big\} \nonumber \\
    % & \forall i \in [k+1,N-2], \exists \nu_{i} \in \mathcal{F}, \forall w_{i} \in \boundeddist, x_{i+1} \in \mathcal{K}, \nonumber \\
    % &\exists \nu_{N-1} \in \mathcal{F}, \forall w_{N-1} \in \boundeddist, x_{N} \in \mathcal{T} \big\} \nonumber \\
    %      &= \big\{x_{k} \in \mathcal{K}: \nonumber \\
    % & \forall i \in [k,N-2], \exists \nu_{i} \in \mathcal{F}, \forall w_{i} \in \boundeddist, x_{i+1} \in \mathcal{K}, \nonumber \\
    % &\exists \nu_{N-1} \in \mathcal{F}, \forall w_{N-1} \in \boundeddist, x_{N} \in \mathcal{T} \big\} \nonumber \\
        % \begin{array}{l}
        %     \exists \nu_{k}\in \mathcal{F}, \forall w_{k}\in \boundeddist, x_{k+1} \in \mathcal{K}, \\
        %     \exists \nu_{k+1}\in \mathcal{F}, \forall w_{k+1}\in \boundeddist, x_{k+2} \in \mathcal{K}, \\
        %     \hfill\vdots\hfill \\
        %     \exists \nu_{N-1}\in \mathcal{F}, \forall w_{N-1}\in \boundeddist, x_{N} \in \mathcal{T} \\
        % \end{array}\big\} \\
        & = \radfull{k} \label{eq:recursion-k-end}
    \end{align}
    which completes the proof.
\end{proof}

In systems for which the disturbance is not affine, i.e.
\begin{equation*}
    \dot{x} = f(x, u, w)
\end{equation*}
the recursion in Theorem \ref{thm:robust-effective-target-recursion} can be altered by replacing $\radfull{k+1} \minkdiff \boundeddist$ with $\mathrm{Pre}(\radfull{k+1})$, where $\mathrm{Pre}(\cdot)$ is the predecessor set \cite{rakovic2006_reach}.
Since many systems can be written in the form \eqref{eq:nonlin-dist}, i.e. with affine disturbances, we do not formally prove the recursion using predecessor sets. 
% \begin{proof}
%     We prove this by induction. Starting with the base case,
%     \begin{align}
%         \targetset_{N-1} \,\cap\, & \reachd(\radfull{N} \minkdiff \boundeddist) \nonumber \\
%         & = \targetset_{N-1} \cap \reachd(\targetset_{N} \ominus \boundeddist) \\
%         & = \targetset_{N-1} \cap \big\{x^{-} \in \statespace : \exists \nu \in \mathcal{F}, \forall w_{N-1} \in \boundeddist \nonumber \\
%         & \hskip2cm f(x^{-}, \nu(x^{-})) + w_{N-1} \in \targetset_{N} \big\} \\
%         & = \big\{ x_{N-1} \in \mathcal{K}: \exists \nu_{N-1} \in \mathcal{F}, \forall w_{N-1} \in \boundeddist, \nonumber \\
%         & \hskip2cm f(x_{N-1}, \nu(x_{N-1})) + w_{N-1} \in \targetset_{N} \big\} \\
%         & = \big\{ x_{N-1} \in \mathcal{K} : \exists \nu_{N-1} \in \mathcal{F}, \forall w_{N-1} \in \boundeddist, \nonumber \\
%         & \hskip2cm x_{N} \in \targetset_{N} \big\} \\
%         & = \radfull{N-1}.
%     \end{align}
%     For any $k \in \naturalnums$, $k < N-1$
%     % , see equations 
%     % \eqref{eq:recursion-k-start}--\eqref{eq:recursion-k-end}.
%     \begin{align}
%         \targetset_{k} \,\cap\, &\reachd(\radfull{k+1} \minkdiff \boundeddist) \nonumber \\
%         & = \big\{ x_{k} \in \targetset_{k}: \exists \nu_{k} \in \mathcal{F}, \forall w_{N-1} \in \boundeddist, \nonumber \\
%         & \hskip1.5cm f(x_{k}, \nu(x_{k})) + w_{N-1} \in \radfull{k+1} \big\} \label{eq:recursion-k-start}\\
%         & = \big\{ x_{k} \in \targetset_{k} : \exists \nu_{k} \in \mathcal{F}, \forall w_{N-1} \in \boundeddist,  \nonumber \\
%         & \hskip1.5cm x_{k+1} \in \radfull{k+1} \big\}.
%     \end{align}
%     By expanding $\radfull{k+1}$ with its definition \eqref{eq:retset},
%     \begin{align}
%         % \phantom{\hbox to 0.8cm{}} &= \left\{ x_{k} \in \mathcal{K} : \exists \nu_{k} \in \mathcal{F}, \forall w_{N-1} \in \boundeddist,  x_{k+1}, \in \left\{x_{t+1} \in \mathcal{K}:
%         % \begin{array}{l}
%         %     \exists \nu_{t+1}\in \mathcal{F}, \forall w_{t+1}\in \boundeddist, x_{t+2} \in \mathcal{K}, \\
%         %     \hfill\vdots\hfill \\
%         %     \exists \nu_{N-1}\in \mathcal{F}, \forall w_{N-1}\in \boundeddist, x_{N} \in \mathcal{T} \\
%         % \end{array}\right\}\right\} \\
%         \phantom{\hbox to 0.89cm{}} & = \left\{  x_{k} \in \mathcal{K} : 
%         \begin{array}{l}
%             \exists \nu_{k}\in \mathcal{F}, \forall w_{k}\in \boundeddist, x_{k+1} \in \targetset_{k+1}, \\
%             \exists \nu_{k+1}\in \mathcal{F}, \forall w_{k+1}\in \boundeddist, x_{k+2} \in \targetset_{k+2}, \\
%             \hfill\vdots\hfill \\
%             \exists \nu_{N-1}\in \mathcal{F}, \forall w_{N-1}\in \boundeddist, x_{N} \in \targetset_{N} \\
%         \end{array}\right\} \\
%         & = \radfull{k} \label{eq:recursion-k-end}
%     \end{align}
%     which completes the proof.
% \end{proof}
% \begin{proof}
%     \todo[inline]{Can't we use Bertsekas way instead of Aubin's? Something like the proof of induction?}
%     The following proof is a restatement of that in \cite{GleasonCDC2017}, updated to incorporate the notion of target tubes.
    
%     We first demonstrate that we can determine the robust reachable set through the recursion
%     \begin{align}
%         \rad_{N}(\targetsete_{N},\boundeddist) &= \targetset_{N} \label{eq:dra_recurs_lem1}\\
%         \rad_{k}(\targettube_{N},\boundeddist) &= \left\{x \in
%             \targetset_{k} : \right. \nonumber\\
%         &\quad \left. \reachf(x) \cap (\rad_{k+1}( \targetset, \safeset) \minkdiff \boundeddist) \neq
%         \emptyset \right\}.\label{eq:dra_recurs_lem2}
%     \end{align}
%     We start the induction at $N-1$
%       \begin{align*}
%     \rad_{N-1}(&\targettube_{N},\boundeddist) = \left\{x \in \statespace :  \exists \nu(\cdot)\in \mathcal{F}, x \in \targetset_{N-1}, \forall w \in \boundeddist, \right. \\
%    &\hskip2cm \left. \exists y\in \targetset_{N}, y=f(x,\nu(x))+w\right\} \\
%     &= \left\{x \in \statespace : x \in \targetset_{N-1}, \exists \nu(\cdot)\in \mathcal{F}, \right.  \nonumber \\
%   &\hskip1cm \exists y\in \left.(\targetset_{N} \minkdiff \boundeddist) , y=f(x,\nu(x))\right\} \\
%              &= \left\{x \in \targetset_{N-1} : \exists y, y \in \reachf(x)
%   \cap y\in (\targetset_{N} \minkdiff \boundeddist) \right\} \\
%              &= \left\{x \in \targetset_{N-1} : \reachf(x) \cap (\rad_{N}(\targettube_{N},\boundeddist) \minkdiff \boundeddist) \neq \emptyset \right\}
%   \end{align*}
%   For any $t\in \mathbb{N}_{[0,N-2]}$, from \eqref{eq:retset},
%   \begin{align}
%       \rad_{t+1}(\targettube_{N},\boundeddist) &= \left\{ x \in \targetset_{t-1} :
%       \exists \rho_{t+1}\in \mathcal{P}_{N-t-1}, \right.\\
%       &\hskip-1cm \left.\forall\bar{w}_{t+1}\in \boundeddist^{N-t-1}, \forall k \in \mathbb{N}_{[t+1,N]}, x_{k} \in \targettube_{N} \right\}.\label{eq:retset-t}
%   \end{align}
%   Using \eqref{eq:retset-t}, we construct $\rad_{t}(\targetset,
%   \safeset, \boundeddist)$ in the form of \eqref{eq:dra_recurs_lem2}.
%   \begin{align}
%       &\rad_{t}(\targettube_{N},\boundeddist) \nonumber \\
%       &= \left\{ x_{t} \in \statespace :
%       \exists \rho_{t}\in \mathcal{P}_{t},\forall \bar{w}_{t}\in
%       \boundeddist^{N_t}, \forall k \in \mathbb{N}_{[t,N]}, \right.\nonumber \\ 
%      &\quad\quad\quad\quad\left. x_{k} \in
%   \targettube_{N} \right\} \nonumber \\
%     &= \left\{ x_{t} \in \statespace : x_{t}\in \targetset_{t}, \exists \nu_{t}(\cdot)\in \mathcal{F}, \exists \rho_{t+1}\in \mathcal{P}_{N-t-1},
%   \right. \nonumber \\
%   &\quad\quad\quad\quad\rho_t=[\nu_t, \rho_{t+1}], \forall
%   w_t\in \boundeddist,\forall \bar{w}_{t+1}\in \boundeddist^{N-t-1}, \nonumber \\
%   &\quad\quad\quad\quad\left.  \forall k \in \mathbb{N}_{[t+1,N]},x_{k}
%         \in \targettube_{N} \right\} \label{eq:prevP1}\\
%             &= \left\{ x_{t} \in \targetset_{t} : \exists \nu_{t}(\cdot)\in \mathcal{F},\forall w_t\in \boundeddist, \exists y\in \rad_{t+1}(\targettube_{N},\boundeddist)\right. \nonumber \\
%             &\left.\quad\quad\quad\quad  y = f(x_t,\nu_t(x_t))+w_t  \right\}
%   \label{eq:nextP1}\\
%             &= \left\{ x_{t} \in \targetset_{t} : \exists \nu_{t}(\cdot)\in
%   \mathcal{F},\exists y\in \rad_{t+1}(\targettube_{N}, \boundeddist)\minkdiff
%     \boundeddist, \right. \nonumber \\
% &\quad\quad\quad\quad\left. y= f(x_t,\nu_t(x_t)) \right\} \nonumber \\
%             &= \left\{x_{t} \in \targetset_{t} : \reachf(x_{t}) \cap
% (\rad_{t+1}(\targettube_{N},\boundeddist) \minkdiff \boundeddist) \neq
% \emptyset \right\}. \nonumber
% \end{align}

% Combining \eqref{eq:dra_recurs_lem2} and \eqref{eq:dFcapS} completes the proof.
% \end{proof}
\begin{lemma}{~\cite[Proposition 3]{bertsekas1971minimax}}
    For the dynamics \eqref{eq:lin}, if $ \inputspace$ is a convex and compact set, the target tube, $\targettube_{N}$, is convex and compact,
    % $\targetset_{t}\ \forall t\in \mathbb{N}_{[1, N]}$ are convex and compact sets, 
    $\boundeddist$ and $\boundeddistover$ are compact sets, and state matrix $A$ in \eqref{eq:lin} is non-singular, then $\rad_{k}( \targettube_{N}, \boundeddist)$ is convex and compact, $\forall k \in \mathbb{N}$.\label{lem:rrscvx}
\end{lemma}
% subsection Recursion for computation of robust reachable set  (end)

The sufficient conditions for convexity established by Lemma \ref{lem:rrscvx} allow for the recursion in Theorem \ref{thm:underapprox} to be implemented by current computational geometry tools.

\subsection{Recursion for computation of augmented effective target set}

\begin{theorem}\label{thm:augmented-effective-target-recursion}
    For the system given in (\ref{eq:nonlin-dist}), the finite-time disturbance-augmented viable set $\radover_{k}$ can be computed using the recursion  for $k\geq,k\in \mathbb{N}$:
    \begin{align}
        \radover_{N}(\targettube_{N},\boundeddistover) &= \targetset_{N} 
        \label{eq:raover_recurse0} \\
        \radover_{k}(\targettube_{N},\boundeddistover) &= \targetset_{k} \cap
            \reachd(\radover_{k+1}( \targettube_{N},\boundeddistover) \minkadd (-\boundeddistover))\label{eq:raover_recursen}
    \end{align}
\end{theorem}
\begin{proof}
    \todo[inline]{Can't we use Bertsekas way instead of Aubin's? Something like the proof of induction?}
\end{proof}
\todo[inline]{Do we need the following block here?
    Note that for affine control systems, $\reachd(\radover_{k+1}( \targettube_{N},\boundeddistover) \minkadd (-\boundeddistover))$ simplifies to $\reachd^+(\radover_{k+1}( \targettube_{N},\boundeddistover))$ where $\reachd^+$ is the one-step backward reach for a system whose control input space is now $B \inputspace \oplus F \boundeddistover$. 
Hence, the name augmented.}
\begin{figure*}
  \begin{center}
    \includegraphics{rra-avs.png}
  \end{center}
  \caption{Graphical representation of Lagrangian methods for computing (a) the robust effective target set $\rad_{k}(\targettube_{N},\boundeddist)$ from $\rad_{k+1}(\targettube_{N},\boundeddistover)$ via \eqref{eq:dra_recursen} and (b) the augmented effective target set via \eqref{eq:raover_recursen}.}
  \label{fig:ra-bound-dist}
\end{figure*}

%\begin{corollary}
    %$\rad_k(\targettube_{N},\boundeddist) \subseteq \targetset_{k}$ and $\radover_k(\targettube_{N},\boundeddistover) \subseteq \targetset_{k}$  $\forall k\geq 1,
    %k\in \mathbb{N}$.\label{corr:Prop2}
%\end{corollary}

%\begin{corollary}
    %When the bounded disturbance is $\boundeddist = \boundeddistover =\{0_{n}\}$, the n-dimensional origin, $\rad_{k}(\targettube_{N},\boundeddist) = \radover(\targettube_{N},\boundeddistover)$.
%\end{corollary}
%[[This is a restatement of something earlier.]]

\begin{lemma}
    For the dynamics \eqref{eq:lin}, if $ \inputspace$ and $\targetset_{t}\ \forall t\in \mathbb{N}_{[1, N]}$ are convex and compact sets, $\boundeddist$ and $\boundeddistover$ are compact sets, and state matrix $A$ in \eqref{eq:lin} is non-singular, then $\radover_{k}( \targettube_{N}, \boundeddist)$ is convex and compact, $\forall k \in \mathbb{N}$.\label{lem:augmented-set-convex-conditions}
\end{lemma}
\begin{proof}
    Has a similar proof to Lemma 1 and uses the fact that Minkowski sums of convex compact sets are convex compact (Citation?).
\end{proof}
% subsection Recursion for computation of robust reachable set  (end)

% \subsection{Minimum volume set theory (may be pushed off)}
% \begin{lemma}
%     If $\boundeddist_1\subseteq\boundeddist_2$, then $\rad( \safeset, \targetset, \boundeddist_2)\subseteq\rad( \safeset, \targetset, \boundeddist_1)$.\label{lem:decWorst}
% \end{lemma}
% \begin{proof}
%     By $\forall \bar{w}_t$ in the definition of $\rad()$. 
% \end{proof}
% We can partition the subsets of $ \distspace^N$ that satisfy the condition $\prob( \overline{w}\in \worstEps)\geq\beta$ into monotone families of sets.
% By Lemma~\ref{lem:decWorst}, each of this monotone family has a minimal set that is a subset of all sets in the family and has the largest robust reach-avoid set generated by the family.
% Thus, we have a set of minimal sets that can serve as $\worstEps$.
% \myni{Some of these robust reach-avoid sets could be empty. That could be used to winnow these chaffs (Help identify additional restrictions on Claim~\ref{cl:MVS}).}
% \begin{cl}
%     If $\vol(\boundeddist_1)\leq\vol(\boundeddist_2)$ (+ some additional conditions), then $\rad(\safeset, \targetset, \boundeddist_1)\subseteq\rad( \safeset, \targetset, \boundeddist_2)$?\label{cl:MVS}
% \end{cl}
% \myni{Without additional conditions, this doesn't look right by Joe's counterexample. We could have $\boundeddist_1$ be a small set very far away (strong distrubance).}
% \myni{JG: Yeah, we definitely can't get subset proof without some more assumptions because of the counterexample that we talked about a while ago. My question is whether or not we can do something like the claim below.}
% \begin{cl}
%   If $\vol(\boundeddist_{1}) \leq \vol(\boundeddist_{2})$ then
%     $\vol(\rad(\safeset, \targetset, \boundeddist_1)) \leq \vol(\rad(\safeset, \targetset, \boundeddist_2))$
% \end{cl}
% \myni{JG: I'm fairly certain that we cannot make Claim 2 generically. There may be some assumptions on $\boundeddist_{1}, \boundeddist_{2}$, and $\rad(\safeset, \targetset, \boundeddist_{i}), i=1,2$, but the crux of the claim would lie under the assumption that $\vol(A\ominus\boundeddist_{2}) \geq \vol(A\ominus\boundeddist{1})$ for some set $A$. This, however, is not true in general. I am uncertain, at this point, what assumptions would be necessary or sufficient to make this true. There are simple counterexamples to demonstrate that even under assumptions of compactness of all sets the above assumption is not valid. We would likely need some sort of relationship between $\boundeddist_{1}$ and $\boundeddist_{2}$.}
% Once we figure out Claim~\ref{cl:MVS}, then we can maybe show that minimum volume set is the way to go as we can compute the minimum volume set among the minimal volume sets given by Lemma~\ref{lem:decWorst}.
% subsection Worst case set is contained in the best case set (end)


% section algorithm_and_challenges (end)

\section{Improving Approximations With Multiple Bounded Sets} % (fold)
\label{sec:improving_approximations_with_multiple_bounded_sets}

In the previous sections we detailed how the robust and augmented effective target
sets can be used to under or overapproximate the stochastic reach-avoid level set.
Here we will detail how utilizing multiple bounded disturbance sets can be
used to improve the approximations, i.e. reduce the conservativeness of the underapproximation
and decrease the size of the overapproximation. These improvements come at the 
increase in computational cost of computing multiple robust or augmented target
sets for many different disturbances. Since these sets are determined via Lagrangian
recursions the computation time is still small compared to other methods.

\subsection{Improving the Robust Effective Target Set} % (fold)
\label{sub:improving_the_robust_effective_target_set}

The algorithms and theorems from this section are restatements of work from 
\cite{gleason_2018}, extended to apply for target tubes instead of specifically
addressing the terminal reach-avoid problem.

\begin{theorem}
    \label{prop:approx-unions}
    Let $\boundeddist_{i}$, be a bounded set which 
    satisfies the condition
    \begin{equation}
        \prob\left(\bar{w}_{[k,N-1]} \in \boundeddist_{i}^{N-k} \right) = \beta
    \end{equation}
    for all $i \in \naturalnums_{[1,M]}$, $\bar{w}_{[k,N-1]} = [w_{k}, w_{k+1}, \dots
    w_{N-1}]$. For a nonlinear system \eqref{eq:nonlin-dist}, the union of each
    robust reach avoid set is a subset of the true reach-avoid level set, i.e.
    \begin{equation}
        \radnl{k}{[1,M]} = \bigcup_{m=1}^{M} \rad_{k}(\targettube_{N}, \boundeddist_{m}) \subseteq \levelset_{k}.
        \label{eq:union-subset}
    \end{equation}
\end{theorem}
\begin{proof}
    From \cite[Theorem 4]{GleasonCDC2017} $\rad_{k}(\targettube_{N},
    \boundeddist_{i}) \subseteq \levelset_{k}$ for each $i \in \integerset_{[1,N]}$.
    Thus the union of these sets remains a subset of $\levelset_{k}$.
\end{proof}

\begin{theorem}
    \label{prop:convex-hull}
    Let $\boundeddist_{i}$, be a bounded set which 
    satisfies the condition
    \begin{equation}
        \prob\left(\bar{w}_{[k,N-1]} \in \boundeddist_{i}^{N-k} \right) = \beta
    \end{equation}
    for all $i \in \naturalnums_{[1,M]}$, $\bar{w}_{[k,N-1]} = [w_{k}, w_{k+1}, \dots
    w_{N-1}]$. For a linear system \eqref{eq:lin}, if $\mathcal{U}$ 
    is convex and compact, $\targettube_{N}$ is closed and convex, 
    and $Q(\cdot|x, u)$ is continuous and log-concave, then 
    the convex hull of the robust reach avoid set for each bounded
    disturbance $\rad_{k}(\targettube_{N}, \boundeddist_{i})$, is a 
    subset of the true reach-avoid level set $\levelset_{k}$, i.e. 
    \begin{equation}
        \radlin{k}{[1,M]} = \mathrm{Co}\big(\bigcup_{m=1}^{M} \rad_{k}(\targettube_{N}, \boundeddist_{m}) \big) \subseteq \levelset_{k}.
        \label{eq:convex-hull-subset}
    \end{equation}
\end{theorem}
\begin{proof}
    From \cite[Theorem 4]{GleasonCDC2017} $\rad_{k}(\targettube_{N},
    \boundeddist_{i}) \subseteq \levelset_{k}$ for each $i \in \naturalnums_{[1,M]}$,
    and from \cite[Theorem 4]{VinodHSCC2018}, $\levelset_{k}$ is convex. Thus, the convex
    hull of robust reach avoid sets is a subset of $\levelset_{k}$ \cite[Section 2.3.4]{BoydConvex2004}.
\end{proof}

\begin{lemma}
    Let $\boundeddist_{j}$ be a bounded set in the collection $\boundeddist_{1}, \dots,
    \boundeddist_{M}$, $M,j \in \naturalnums$, $j < M$. Then
    \begin{equation}
        \rad_{k}(\targettube_{N}, \boundeddist_{j}) \subseteq \radlin{k}{[1,M]}
    \end{equation}
\end{lemma}
\begin{proof}
    For a nonlinear system \eqref{eq:nonlin-dist}, for any $x \in \rad_{k}(\targettube_{N}, \boundeddist_{j})$, 
    $x \in \radnl{k}{[1,M]}$ by \eqref{eq:union-subset}, and for a linear system \eqref{eq:lin} 
    any $y \in \rad_{k}(\targettube_{N}, \boundeddist_{j})$, 
    $y \in \radlin{k}{[1,M]}$ by \eqref{eq:convex-hull-subset}.
\end{proof}
\begin{algorithm}[]
    \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}

    \Input{Target tube $\targettube$; system dynamics; desired probability level $\beta \in [0,1]$; $M$ bounded
    disturbance sets, $\boundeddist_{1},\dots,\boundeddist_{M}$; horizon length, $N$}
    \Output{$N$-time stochastic reach-avoid $\beta$-level set underapproximation, $\radnl{0}{[1,M]}$}
    \vskip6pt
 % \KwData{this text}
 % \KwResult{how to write algorithm with \LaTeX2e }
%     Compute $\boundeddist$ for $\beta^{\frac{1}{N}}$ \hfill // from (\ref{eq:ellipsoid}), (\ref{eq:R2}) \\
    % \For{$m = 1, 2, \dots, M$}{
    %     $\rad_{N}(\mathcal{K},\mathcal{T},\boundeddist_{m}) \leftarrow \mathcal{T}$
    % }
    
    $\rad_{N}(\targettube_{N}, \boundeddist_{m}) \leftarrow \mathcal{T}_{N}$, $\forall m \in \mathbb{N}_{[1,M]}$ \\
    % $\radimproved{N}{[1,M]} \leftarrow \mathcal{T}$ \\
    \For{$i = N-1, N-2, \dots, 0$}{
        \For{$m = 1, 2, \dots, M$}{
            // from \eqref{eq:dra_recursen} \\
            $S \leftarrow \rad_{i+1}(\mathcal{K},\mathcal{T},\boundeddist_{m}) \minkdiff \boundeddist_{m}$ \\
            $E \leftarrow \reachd(S)$ \\
            $\rad_{i}(\targettube_{N}, \boundeddist_{m}) \leftarrow \mathcal{T}_{k} \cap E$ \hfill \\
        }
        
        \If{nonlinear system dynamics \eqref{eq:nonlin-dist}}{
            $\radnl{i}{[1,M]} \leftarrow 
        \bigcup_{m=1}^{M}\rad_{i}(\targettube_{N}, \boundeddist_{m})$
        }

        \If{linear system dynamics \eqref{eq:lin}}{
            $\radlin{i}{[1,M]} \leftarrow 
        \mathrm{Co}\big(\bigcup_{m=1}^{M}\rad_{i}(\targettube_{N}, \boundeddist_{m})\big)$
        }
    }
    \caption{Underapproximation of the $N$-time stochastic effective $\beta$-level set using multiple bounded disturbances and unions.}
    \label{alg:union-algorithm}
\end{algorithm}

% subsection improving_the_robust_effective_target_set (end)

\subsection{Improving the Augmented Effective Target Set} % (fold)
\label{sub:improving_the_augmented_effective_target_set}

\begin{theorem}
    \label{prop:approx-unions}
    Let $\boundeddistover_{i}$, be a bounded set which 
    satisfies the condition
    \begin{equation}
        \prob\left(\bar{w}_{[k,N-1]} \in \boundeddistover_{i}^{N-k} \right) = \beta
    \end{equation}
    for all $i \in \naturalnums_{[1,M]}$, $\bar{w}_{[k,N-1]} = [w_{k}, w_{k+1}, \dots
    w_{N-1}]$. For a nonlinear system \eqref{eq:nonlin-dist}, the union of each
    robust reach avoid set is a subset of the true reach-avoid level set, i.e.
    \begin{equation}
        \radovernl{k}{[1,M]} = \bigcap_{m=1}^{M} \radover_{k}(\targettube_{N}, \boundeddistover_{m}) \supseteq \levelset_{k}.
        \label{eq:intersection-subset}
    \end{equation}
\end{theorem}
\begin{proof}
    From \cite[Theorem 4]{GleasonCDC2017} $\radover_{k}(\targettube_{N},
    \boundeddistover_{i}) \supseteq \levelset_{k}$ for each $i \in \integerset_{[1,N]}$.
    Thus the intersection of these sets remains a subset of $\levelset_{k}$.
\end{proof}

\begin{lemma}
    Let $\boundeddistover_{j}$ be a bounded set in the collection $\boundeddistover_{1}, \dots,
    \boundeddistover_{M}$, $M,j \in \naturalnums$, $j < M$. Then
    \begin{equation}
         \radovernl{k}{[1,M]} \subseteq \radover_{k}(\targettube_{N}, \boundeddistover_{j})
    \end{equation}
\end{lemma}
\begin{proof}
    % For a nonlinear system \eqref{eq:nonlin-dist} or linear system \eqref{eq:lin}, for any $x \in \radovernl{k}{[1,M]}$, $x \in \radover_{k}(\targettube_{N}, \boundeddistover_{j})$ by \eqref{eq:intersection-subset}. 
    From the intersection operation in \eqref{eq:intersection-subset}, clearly
    $\radovernl{k}{[1,M]} \subseteq \radover_{k}(\targettube_{N}, \boundeddistover_{j})$
    for any $j \in \{1, \dots, M\}$.
\end{proof}

% subsection improving_the_augmented_effective_target_set (end)

% subsection improving_approximations_with_multiple_bounded_sets (end)

\section{Numerical computation}
\label{sec:numerical_computation}

Since Lagrangian methods are grid-free, they have the potential to provide substantial numerical benefits, most notably a dramatically increased computational speed and applicability to high-dimensional systems.
However, the current tools available for numerical computation of the robust reach-avoid sets and augmented viable sets limit its deployability at present.
There are a number of computational challenges that must be faced when applying Lagrangian methods to high-dimensional systems.

One primary challenge is that many of the current toolboxes for computational geometry do not support the necessary set operations for the robust reach-avoid and augmented viable sets.
In particular, the implementation of the Minkowski (Pontryagin) difference operation is an often unsupported operation. 
For support vectors, this difference can be computed against $\mathcal{H}$-polytopes [ref] but there is no closed form expression using only support functions.

Two toolboxes, MPT and the Ellipsoidal toolbox [refs], can support all of the necessary set operations however the Ellipsoidal toolbox adds an additional layer of conservatism to the results since all sets must be represented as ellipsoids,
For example, intersection operations must be underapproximated as an ellipse since the intersection between two ellipses is not necessarily an ellipse.
The Multi-Parametric Toolbox also supports all necessary set operations---and all examples in this paper utilize this toolbox---however because MPT utilizes both vertex and facet representations of polytopes to solve various set operations, it must commonly solver the vertex-facet enumeration problem, which is a complex problem for high-dimensional polytopes. 
Additionally high-dimensional polytopes become increasingly complicated to represent using vertex or facet representation, demanding more memory and processing recourses.

Another difficult problem for high-dimensional systems is in the representation of the bounded disturbance. 
From \cite{GleasonCDC2017}, it is easy to determe a closed-form expression for the bounded disturbance ellipse when the disturbance is from a Gaussian distribution. 
However representing this ellipse can be problematic.
In order to obtain a good approximation of the ellipse using either facet polytope representation or support function representation we would like to choose $m$ directions in $n$ dimensional space that are equidistant, i.e. $x_{i}^{T}x_{j} = k$ for all $i \neq j$, $k$ is some constant.
Choosing equidistant vectors eliminates the possibility of creating unbounded or very large overapproximations of the ellipsoid from poor directional choice; instead unboundedness or large overapproximations would arise if $m$ is very small, especially compared to the dimension size $n$, e.g. if $m < n$.
For a two-dimensional system choosing the appropriate directions is a simple problem in which $x_{i}^{T}x_{j} = cos(2*pi/m)$, see Figure \ref{fig:ellipse-approximatinos}.
\begin{figure}
  \centering
  \includegraphics{figures/ellipse-approxes.png}
  \caption{Ellipsoid approximations from (a) random directions (b) equidistant vector generation, $n = 2$, $m = 8$.}
  \label{fig:ellipse-approximatinos}
\end{figure}
In systems with $n>2$, however, there are some suggested methods for choosing directions [[I think we had a ref or two about this]], but these methods are heuristic and do not necessary provide equidistant vectors.

\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline                                  % For the horizontal line above. 
    Property & H-polytope & V-polytope & $h(L)$ & $\sigma()$ & Star \\ \hline
    Linear transformation & & & & &  \\ \hline
    Minkowski sum & & & & & \\ \hline
    Minkowski difference & & & & &  \\ \hline
    Intersection & & & & & \\ \hline
   \end{tabular}
   \caption{Set-theoretic operations using various representation}
   \label{tab:setrep}
\end{table}

\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline                                  % For the horizontal line above. 
    Property & MPT & SpaceEx & HyLAA & CORA & Flow \\ \hline
    Linear transformation & & & & &  \\ \hline
    Minkowski sum & & & & & \\ \hline
    Minkowski difference & & & & &  \\ \hline
    Intersection & & & & & \\ \hline
   \end{tabular}
   \caption{Set-theoretic operations using various toolboxes (Not going to be included because chances are we might to do a shoddy job and shoot ourselves in the foot)}
   \label{tab:setrep}
\end{table}

% subsection Numerical computation (end)




==> extras.tex <==
\subsection{Bertskas' formulation for the set $ \mathcal{C}()$}
\myni{@Abraham: Update this section to obtain a min-min problem.}

Note that a max-min formulation for $\rad$ was provided in~\cite{GleasonCDC2017}.
The Bertsekas formulation of the set $ \mathcal{C}()$ is a similar setup with maximize over $\rho_t$ and minimize over $w_t$,
\begin{align}
  \begin{array}{rl}
      \underset{\rho_{t}}{\mbox{maximize}}&\hskip-0.3cm\underset{\bar{w}_{t}}{\mbox{
      minimize}}\  L(\rho_{t-1},\bar{w}_{t-1};x_0,t)=\sum_{k=0}^{t} g_k(x_k) \\
     %t-\left(\sum_{k=0}^{t-1} \ONE_{\safeset}(x_k)\right)-\ONE_{\targetset}(x_t)  \\
      \mbox{subject to}& \hskip-0.2cm\left\{\arraycolsep=2pt \begin{array}{rl}
      x_{k+1} &= f(x_k,\nu_k(x_k))  +w_k\\
      w_k & \in \boundeddist \\
      \nu_k(\cdot) & \in \mathcal{F} \\
      %x_0&\in \statespace
      %\bar{w}_{t-1} & =[w_0\ \ldots\ w_{t-1}] \\
      %\rho_{t-1} & =[\nu_0(\cdot)\ \ldots\ \nu_{t-1}(\cdot)] \\
    \end{array}\right., \hskip0.4cm k \in \mathbb{N}_{[0,t-1]}
  \end{array}
  \label{eq:prob-minmax}
\end{align}
where the decision variables are $ \rho_t$ and $\bar{w}_t$. 
Here, $g_k(\cdot)=1-\ONE_{\safeset}(\cdot)$ for $k\in \mathbb{N}_{[0,t-1]}$  and $g_t(\cdot)=1-\ONE_{\targetset}(\cdot)$. 
The objective function $L(\cdot)$ is parameterized by the initial state $x_0\in \statespace$ and the time horizon $t\in \mathbb{N}$. 
Problem \eqref{eq:prob-minmax} can be solved using dynamic programming~\cite[Sec 1.6]{bertsekasDP} to generate the value functions $L^\ast_k(x;t): \statespace \rightarrow \mathbb{N}_{[0,t-k+1]}$ for $k\in \mathbb{N}_{[0,t]}$
\begin{align}
    H^\ast_{k}(u,x;t)&=\inf_{w\in \boundeddist}
    \left[L^\ast_{k+1}(f(x,u)+w;t)+g_k(x)\right]\label{eq:minmaxVH}\\
    L^\ast_k(x;t)&=\sup_{u\in \inputspace}H^\ast_{k}(u,x;t) \label{eq:minmaxV}
\end{align}
initialized with $L^\ast_t(x;t)=g_t(x)$. 
The optimal value of problem \eqref{eq:prob-minmax} when starting at $x_0$ is $L^\ast_0(x_0;t)$. 

% subsection Bertskas' formulation form $ \mathcal{C}()$ (end)




